Deep Bayesian Active Learning for Natural Language Processing: Results of a Large-Scale Empirical Study

Several recent papers investigate Active Learning (AL) for mitigating the data dependence of deep learning for natural language processing. However, the applicability of AL to real-world problems remains an open question. While in supervised learning, practitioners can try many different methods, evaluating each against a validation set before selecting a model, AL affords no such luxury. Over the course of one AL run, an agent annotates its dataset exhausting its labeling budget. Thus, given a new task, an active learner has no opportunity to compare models and acquisition functions. This paper provides a large scale empirical study of deep active learning, addressing multiple tasks and, for each, multiple datasets, multiple models, and a full suite of acquisition functions. We find that across all settings, Bayesian active learning by disagreement, using uncertainty estimates provided either by Dropout or Bayes-by Backprop significantly improves over i.i.d. baselines and usually outperforms classic uncertainty sampling.

==> sections/acquisition.tex <==
In this work, we consider only uncertainty based acquisition. 
In particular, we consider least confidence (LC) for classification and maximum length-normalized log probability (MNLP) for sequence labeling tasks \citep{shen2018deep}. 
Our Bayesian acquisition functions 
are based on the Bayesian Active Learning by Disagreement (BALD) approach due to \citet{houlsby2011bayesian}.
We denote Monte Carlo Dropout Disagreement by DO-BALD and its Bayes-by-Backprop 
counterpart as  BB-BALD.

\paragraph{LC} It involves choosing the samples with lowest confidence assigned by the model. This confidence could be given by the softmax output in neural network. We use this acquisition function for classification task.
\paragraph{MNLP} For sequence labeling tasks, LC disproportionately selects longer sentences because in log scale, LC contains summation over words. Our budget for sequence learning tasks is based on number of words labeled rather than number of sentences because longer sentence require more labour. Therefore, following \cite{DBLP:journals/corr/ShenYLKA17}, we normalize the log probability by length of sentence. Thus the samples are selected according to following criteria:
\begin{equation*}
\argmin_{j} \Big( \max_{y_1^j,..,y_n^j} \frac{1}{n} \sum_{i=1}^n \log \mathbb{P}[y_i^j|y_1^j,.. y_{i-1}^j, \{x_i^j\}] \Big)
\end{equation*}
where $y_i^j$ is the tag of the $ith$ word in $jth$ sample. We use this acquisition for both NER and SRL tasks. 

\paragraph{DO-BALD}
BALD originally selects samples that maximise the information gained about the model parameters. This boils down to choosing data points which each stochastic forward pass through the model would have the highest probability assigned to a different class. \cite{gal2017deep}. Our measure of uncertainty is the fraction of $T$ models with different dropout masks which disagreed with most popular choice. The ties are resolved by the mean of output probability of $T$ models.
\begin{equation*}
\argmax_j \left( 1 - \frac{count(mode(y_j^{(1)},..., y_j^{(t)})}{T}) \right)
\end{equation*}
This can be easily extended to sequences by taking the count of mode of entire sequence instead of words. In our work, this has been used both for classification and sequence labeling.

\paragraph{BB-BALD}
Instead of the different dropout masks, the disagreement is between the outputs of different weights in the network which are sampled from a Gaussian. It is important to note here that BB model is used only for acquisition of samples and for training we use standard models and the two are trained concurrently.
